Rewrite based Verification of XML Updates

We consider problems of access control for update of XML documents. In the context of XML programming, types can be viewed as hedge automata, and static type checking amounts to verify that a program always converts valid source documents into also valid output documents. Given a set of update operations we are particularly interested by checking safety properties such as preservation of document types along any sequence of updates. We are also interested by the related policy consistency problem, that is detecting whether a sequence of authorized operations can simulate a forbidden one. We reduce these questions to type checking problems, solved by computing variants of hedge automata characterizing the set of ancestors and descendants of the initial document type for the closure of parameterized rewrite rules.

==> README <==
README for rr-inria as of 09-07-2009 

Il y a trois repertoires dans l'archive: inputs latex logos
Le repertoire inputs contient les deux fichiers RR.dtx et RR.ins 
qui permetttent de construire les fichiers de style et la documentation. 
Le repertoire latex contient les fichiers de style et la documentation.
Le repertoire logos contient l'ensemble des logos des divers 
centres (et unites) de recherche. 
Ces logos sont identiques a ceux distribues en decembre 2007.

Il convient de mettre les fichiers de style dans un repertoire reconnu par 
latex, et les logos dans un repertoire reconnu par pdflatex (en cas de 
production directe du pdf) ou par latex et dvips (en cas de production d'un 
fichier PostScript intermediaire). Si on veut deposer les source d'un rapport 
Inria sur HAL, il faut egalement deposer le fichier de style et les logos 
utilises.

Nouveau. Les commandes \RRtheme et \RRdomaine permettent de specifier 
le theme ou le domaine de rechereche de l'equipe.


------------------------------------------------

This package contains three folders: inputs latex logos
The inputs folder contains the two files RR.ins and RR.dtx that can be used 
to produce the style files and the documentation.
The latex folder contains the style file and and the folders.
The logos folder contains the logos used for the research units and centers.
The logos are the same as those ditributed sincve December 2007.

You should put the style files into a folder where latex looks for style file.
You should put the logos in a folder serach by pdflatex (for dirtect production
of Pdf) or latex and dvips (when an intermediate PostScript file is generated).
If you want to put the sources of the report on HAL, do not forget to upload 
the style file as well as the requirted logos.

New: The two commands \RRtheme and \RRdomaine can be used to indicate 
the Theme or Domain of the Team.


